Testing Determinantal Point Processes

Determinantal point processes (DPPs) are popular probabilistic models of diversity. In this paper, we investigate DPPs from a new perspective: property testing of distributions. Given sample access to an unknown distribution $q$ over the subsets of a ground set, we aim to distinguish whether $q$ is a DPP distribution, or $\epsilon$-far from all DPP distributions in $\ell_1$-distance. In this work, we propose the first algorithm for testing DPPs. Furthermore, we establish a matching lower bound on the sample complexity of DPP testing. This lower bound also extends to showing a new hardness result for the problem of testing the more general class of log-submodular distributions.

==> learner-sv.tex <==
\def\Kt{\Tilde{K}}



\section{An Algorithm for Testing DPPs} \label{sec:learning}
We will first construct an algorithm for testing the smaller class of $(\alpha,\zeta)$-normal DPPs, and then show how to extend this result to all DPPs via a coupling argument.

Our testing algorithm relies on learning: given samples from $q$, we estimate a kernel $\hat K$ from the data, and then test whether the estimated DPP has generated the observed samples. The magnitude of any entry $\hat{K}_{i,j}$ can be estimated from the marginals for $S = \{i,j\}$ and $i,j$, since $\dpp{K}{S} = K_{i,i}K_{j,j} - K_{i,j}^2 = \dpp{K}{i}\dpp{K}{j} - K_{i,j}^2$. But, determinig the signs is more challenging. \citet{urschel2017learning} estimate signs via higher order moments that are harder to estimate, but it is not clear whether the resulting estimate $\hat{K}$ yields a sufficiently accurate estimate of the distribution to obtain an optimal sample complexity for testing.
Hence, instead, we construct a set $\MM$ of candidate DPPs such that, with high probability, there is a $\tilde p \in \mathcal M$ that is close to $q$ if and only if $q$ is a DPP. Our tester, Algorithm~\ref{alg:testing_DPP}, tests closeness to $\MM$ by individually testing closeness of each candidate in $\MM$.

\begin{algorithm}[t]
\caption{\dpptester \label{alg:testing_DPP}}
\begin{algorithmic}[1]
\Procedure{DPP-Tester}{$\epsilon$, $\delta$, sample access to $q$}
    \State{$\MM \gets $ construct the set of DPP distributions as described in Theorem~\ref{thm:learning}.}
    \For {each $p$ in $\MM$}
        \State{Use robust $\chi^2-\ell_1$ testing to check if $\chi^2(q,p) \leq \epsilon^2/500$, or $\ell_1(q,p) \geq \epsilon$}.
        \If{the tester outputs \accept}
            \State{\textbf{Return} \accept.}
        \EndIf
    \EndFor
 	\State{\textbf{Return} \reject}
\EndProcedure
\end{algorithmic}
\end{algorithm}



\textbf{Constructing $\MM$.} The DPPs in $\MM$ arise from variations of an estimate for $K^*$, obtained with $\Theta(\sqrt N/\epsilon^2)$ samples. Via the above stragegy, we first estimate the magnitude $|K^*_{ij}|$ of each matrix entry, and then pick candidate entries from the confidence intervals around $\pm|\widehat{K}_{ij}|$, such that at least one is close to the true $K^*_{i,j}$. The candidate matrices $K$ are obtained by all possible combinations of candidate entries. Since these are not necessarily valid marginal kernels, we project them onto the positive semidefinite matrices with eigenvalues in $[0,1]$. Then, $\MM$ is the set of all DPPs parameterized by these projected candidate matrices $\Pi(K)$.


If $q$ is a DPP with kernel $K^*$, then, by construction, our candidates contain  a $\tilde{K}$ close to $K^*$. The projection of $\tilde K$ remains close to $K^*$ in Frobenius distance. We show that this closeness of the matrices implies closeness of the corresponding distributions $q$ and $\tilde p = \Pr[\Pi(\tilde K)]{.}$ in $\ell_1$-distance: $\ell_1(q,\tilde p) = O(\epsilon)$. Conversely, if $q$ is $\epsilon$-far from being a DPP, then it is, by definition, $\epsilon$-far from $\MM$, which is a subset of all DPPs. 


\textbf{Testing $\MM$.} To test whether $q$ is close to $\MM$, a first idea is to do robust $\ell_1$ identity testing, i.e., for every $p \in \mathcal M$, test whether $\ell_1(q,p) \geq \epsilon$ or $\ell_1(q,p) = O(\epsilon)$. But, $\MM$ can contain the uniform distribution, and it is known that robust $\ell_1$ uniformity testing needs $\Omega(N/\log N)$ samples~\cite{VV11}, as opposed to the optimal dependence $\sqrt N$.

Hence, instead, we use a combination of $\chi^2$ and $\ell_1$ distances for testing, and test $\chi^2(q,p) = O(\epsilon^2)$ versus $\ell_1(q,p) \geq \epsilon$ \citep{ADK15}. To apply this robust $\chi^2$-$\ell_1$ identity testing, we must prove that, with high probability, there is a $\tilde{p}$ in $\MM$ with $\chi^2(q,\tilde p) = O(\epsilon^2)$ if and only if $q$ is a DPP. Theorem~\ref{thm:learning}, proved in Appendix~\ref{app:appendixa}, asserts this result if $q$ is an $(\alpha, \zeta)$-normal DPP. This is stronger than its $\ell_1$ correspondent, since $\frac{1}{2}\ell_1^2(q,\tilde p) \leq \chi^2(q,\tilde p)$. 

To prove Theorem~\ref{thm:learning}, we need to control the distance between the atom probabilities of $q$ and $\tilde p$. We analyze these atom probabilities, which are given by determinants, via a lower bound on the smallest singular values $\sigma_n$ of the family of matrices $\{ K - I_{\bar J}: \ J \subseteq [n] \}$.
\begin{lemma} \label{smallest-singular-value-lemma}
If the kernel matrix $K$ has all eigenvalues in $[\zeta, 1 - \zeta]$, then, for every $J \subseteq [n]$:
$$\sigma_n(K - I_{\bar J}) \geq \zeta (1 - \zeta)/\sqrt 2.$$
\end{lemma}
%
Lemma~\ref{smallest-singular-value-lemma} is proved in Appendix~\ref{app:appendixb}. In Theorem~\ref{thm:learning}, we observe $m = \lceil (\ln(1/\delta) +  1)\sqrt{N}/\epsilon^2\rceil$ samples from $q$, and use the parameter $\varsigma \coloneqq \lceil 200 n^2\zeta^{-1}  \min\{2\xi/\alpha, \sqrt{\xi/\epsilon} \} \rceil$, with $\xi \coloneqq N^{-\frac{1}{4}} \sqrt{\log(n) + 1}$. 
%
\begin{theorem} \label{thm:learning}
Let $q$ be an $(\alpha, \zeta)$-normal DPP distribution with marginal kernel $K^*$. Given the parameters defined above, suppose we have $m$ samples from $q$. 
Then, one can generate a  set $\mathcal{M}$ of DPP distributions with cardinality $|\mathcal{M}| = (2\varsigma+1)^{n^2}$, such that, with probability at least $1 - \delta$, there is a distribution $\tilde p \in \mathcal{M}$ with $\chi^2(q,\tilde p) \leq \epsilon^2/500$. 
\end{theorem}



\iffalse
  We sketch our testing approach here. Suppose we have sample access to a distribution $q$ over $2^{[n]}$. Our tester relies on learning a marginal kernel matrix $\hat K$ entry by entry from the data, and based on that, generating a family of DPP distributions $\mathcal M$ as potential estimates for $q$, such that if $q$ happens to be a DPP, then there is a particular $\tilde p \in \mathcal M$ close enough to $q$. The algorithm then tries to distinguish the case when $q$ is a DPP from when it is $\epsilon$-far from all DPPs by searching for such a close $\tilde p$ in $\mathcal M$, because if $q$ is not a DPP, then all distributions in $\mathcal M$, which are DPP, are $\epsilon$-far from $q$. This means that when $q$ is a DPP, in order for $\tilde p$ to be distinguishable, it should be at least $\epsilon$-close to $q$. As we noted in section~\ref{sec:mainresults}, if $q$ is a DPP with marginal kernel $K^*$, then producing a $\hat K$ accurate enough, such that $\Pr[\hat K]{.}$ and $q$ are $\epsilon$-close, might not be feasible with $\Theta(\sqrt N/\epsilon^2)$ samples. To obtain more accurate estimates with $\Theta(\sqrt N/\epsilon^2)$ samples, we use the initial estimate $\hat K$, but for each entry $\hat K_{i,j}$, we consider a set of candidates in the confidence interval around $\hat K_{i,j}$ and make sure at least one of them is close enough to $K^*_{i,j}$.
  
  Then, we form a set $M$ of matrices by considering every combination of the candidate values among all the entries. This way, we are confident that there is a $\tilde{K} \in M$ which is close enough to $K^*$ at every entry. Since $\tilde K$ might not be a valid marginal kernel, we consider $\Pi(\tilde K)$, its projection onto the set of positive semi definite matrices $S^n_+$ with eigenvalues in the range $[0,1]$, and we show that $\Pi(\tilde K)$ remains close to $K^*$ in the Frobenius distance. Defining $\tilde p = \Pr[\Pi(\tilde K)]{.}$, we show that closeness of $K$ and $\Pi(\tilde K)$ in the Frobenius distance leads to $\ell_1(q,\tilde p) = O(\epsilon)$. As a result, it is now natural to define the set $\mathcal M$ to be $\{ \Pr[\Pi(K)]{.}: \, K \in M \}$. 
  
 


Given the set $\mathcal M$, to find out if a distribution $\tilde p$ close to $q$ in $\mathcal M$ exists, one might be tempted to perform a robust $\ell_1$ testing for every $p \in \mathcal M$, which is simply a test to distinguish between the cases $\ell_1(q,p) \geq \epsilon$ versus $\ell_1(q,p) = O(\epsilon)$.
However, it is known that testing whether a distribution over $[N]$ is $\epsilon$-close to the uniform distribution, or $(0.5-\epsilon)$-far from the uniform distribution for a constant $\epsilon$, requires $\Omega(N/\log N)$ samples~\cite{VV11}. So robust $\ell_1$ testing requires $\Omega(N /\log N)$ samples in the worst case, while our lower bound suggests that the optimal dependence on $N$ might be of order $\sqrt N$. 

Using the same number of samples, it turns out that one can prove a stronger guarantee for $\tilde p$, namely $\chi^2(q,\tilde p) = O(\epsilon^2)$. Note that $\chi^2$ distance is generally a more restrictive distance measure compared to the squared $\ell_1$ distance, as we have the inequality $\frac{1}{2}\ell_1^2(q,\tilde p) \leq \chi^2(q,\tilde p)$. Having this new bound in hand, we apply the robust $\chi^2-\ell_1$ identity testing, a method proposed by~\citet{ADK15}, which enables us to distinguish the case $\chi^2(q,p) = O(\epsilon^2)$ from $\ell_1(q,p) \geq \epsilon$, with only $O(\sqrt N / \epsilon^2)$ samples. Using the $\chi^2-\ell_1$ test for every $p \in \mathcal M$, we can finally find out if a $\tilde p \in \mathcal M$ with $\chi^2(q,\tilde p) \leq O(\epsilon)$ exists, or $\ell_1(q,p) \geq \epsilon$ for all $p \in \mathcal M$, and consequently figure out if $q$ is a DPP or not.

We formalize our $\chi^2$ distance guarantee for the generated set $\mathcal M$ in Theorem~\ref{thm:learning}, which we exploit later on in section~\ref{sec:mainresults} to prove the correctness of our DPP testing algorithm. For the formal definition of $\hat K$ and $\mathcal M$, see the proof of Theorem~\ref{thm:learning} in Appendix~\ref{app:appendixa}.
Before stating Theorem~\ref{thm:learning}, we state Lemma~\ref{smallest-singular-value-lemma} (proved in Appendix~\ref{app:appendixb}), which is an important building block in bounding $\chi^2(q,\tilde p)$; it testifies a uniform lower bound on the singular values of the family of matrices $\{ K - I_{\bar J}: \ J \subseteq [n] \}$. Recall from Equation~\ref{eq:atomprobabilities}, that the determinant of these matrices gives the atom probabilities of a DPP distribution. We use this singular value lower bound to control the distance between the atom probabilities of $q$ and $\tilde p$.




\begin{lemma} \label{smallest-singular-value-lemma}
Suppose the eigenvalues of a marginal kernel matrix $K$ are in the range $[\zeta, 1 - \zeta]$. Then, for every $J \subseteq [n]$:
$$\sigma_n(K - I_{\bar J}) \geq \frac{\zeta (1 - \zeta)}{\sqrt 2},$$
\end{lemma}
where $\sigma_n(.)$ is the smallest singular value.



Before formally stating the theorem, we set our parameters as follows: Let $N \coloneqq 2^n$ be the domain size of $q$. 
Assume $\epsilon$ and $\delta$ denotes the proximity parameter and the confidence parameter respectively, and $m$ indicates the number of samples from $q$ which we set to be $m = \lceil (\ln(1/\delta) +  1)\sqrt{N}/\epsilon^2\rceil$. We define two parameters $\varsigma$ and $\xi$ as follows: 
\begin{align}
\varsigma \coloneqq \lceil 200 n^2\zeta^{-1}  \min\{\frac{2\xi}{\alpha}, \sqrt{\frac{\xi}{\epsilon}} \} \rceil\,, \ \ \ \  \xi \coloneqq N^{-\frac{1}{4}} \sqrt{\log(n) + 1}\,. \label{eq:epsilonprime}   
\end{align}



\begin{theorem} \label{thm:learning}
Let $q$ be an $(\alpha, \zeta)$-normal DPP distribution with marginal kernel $K^*$. Given the parameters defined above, suppose we have $m$ samples from $q$. 
Then, one can generate a  set $\mathcal{M}$ of DPP distributions with cardinality $|\mathcal{M}| = (2\varsigma+1)^{n^2}$, such that with probability at least $1 - \delta$, there is a distribution $\tilde p \in \mathcal{M}$ with $\chi^2(q,\tilde p) \leq \frac{\epsilon^2}{500}$. 
\end{theorem}

\fi


